Sampling for Remote Estimation of the Wiener Process over an Unreliable Channel

In this paper, we study a sampling problem where a source takes samples from a Wiener process and transmits them through a wireless channel to a remote estimator. Due to channel fading, interference, and potential collisions, the packet transmissions are unreliable and could take random time durations. Our objective is to devise an optimal causal sampling policy that minimizes the long-term average mean square estimation error. This optimal sampling problem is a recursive optimal stopping problem, which is generally quite difficult to solve. However, we prove that the optimal sampling strategy is, in fact, a simple threshold policy where a new sample is taken whenever the instantaneous estimation error exceeds a threshold. This threshold remains a constant value that does not vary over time. By exploring the structure properties of the recursive optimal stopping problem, a low-complexity iterative algorithm is developed to compute the optimal threshold. This work generalizes previous research by incorporating both transmission errors and random transmission times into remote estimation. Numerical simulations are provided to compare our optimal policy with the zero-wait and age-optimal policies.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/Untitled.tex <==
\mathbb{E} \left[ Y \right]

\text{mse}_{\text{opt}}

\sum_{j=1}^{\infty}

\begin{align}

\end{align}

{\large $\mathbbm{1}$}
${\text{\large $\mathbbm{1}$}}_e$

{\text{\large $\mathbbm{1}$}}_{|w+W_{Y_1}|>v_n} 

 \frac{\partial^2}{\partial w^2} 
 
 \frac{d^3}{dw^3}
 
 
 {\text{\large $\mathbbm{1}$}}_{|w| \ge v_{n+1} } 

==> sections/abstract.tex <==
%\IEEEtitleabstractindextext{%
\begin{abstract}
%In this paper, we study the problem of minimizing age-penalty functions at a remote destination by controlling the sample times at the data source. 
%The freshly sampled data is forwarded to the destination through an unreliable channel and the feedback is then sent backward. Both the forward and backward transmission times are random. We formulate a problem of remote estimation using Kalman Filter and show that the related performance metric is a function of the age. For general age-penalty functions, we aim to design an online sampling policy to optimize these data freshness metrics. Motivated by the earlier works, our problem is equivalent to a decomposed problem regarding the time duration between two successful receptions. However, the decomposed problem is still a Markov Decision Process (MDP), which is significantly different from the previous studies and faces the curse of dimensionality. We show that the optimal sampling policy is threshold-based. The threshold is equal to the optimal objective value and is computed by a low complexity bisection algorithm. 
%An interesting consequence is that the optimal policy postpones transmission only if the source receives positive feedback. 
%Numerical simulations are provided to compare with other different sampling policies.  
                          
%In this paper, we study a sampling problem, where freshly sampled data is sent to a remote destination via an unreliable forward channel, and acknowledgments are sent back on a feedback channel. Both the forward and feedback channels are subject to random transmission times. We optimize the sampling strategy at the source (e.g., a sensor) to enhance the freshness of data samples delivered to the destination (e.g., an estimator). This sampling problem is also motivated by a distributed sensing system, where an estimator estimates a signal by combining noisy signal observations collected from a local sensor and accurate signal samples received from a remote sensor. We show that the optimal estimation error is an increasing function of the age of received signal samples. For general non-decreasing age penalty functions, an exact solution to the optimal sampling problem is derived. When the previous transmission succeeded, the source waits until the expected age penalty upon delivery is no smaller than a threshold, then sends the next sample out. The threshold is equal to the optimal objective value and can be calculated by low-complexity bisection search and fixed-point iterations. When the previous transmission failed, no waiting time should be added. 

%In this paper, we study a sampling problem, in which freshly sampled data is sent to a remote destination via an unreliable channel, and acknowledgments are sent back on a reverse channel. Both the forward and feedback channels are subject to i.i.d. random transmission times, whereas the forward channel also suffers from i.i.d. transmission failures. We optimize the sampling strategy at the source (e.g., a sensor), aiming to enhance the freshness of data samples delivered to the destination (e.g., an estimator). This sampling problem is motivated by a distributed sensing system, where an estimator estimates a signal in real-time by combining noisy signal observations collected from a local sensor and accurate signal samples received from a remote sensor. We show that the optimal estimation error is an increasing function of the age of received signal samples. The optimal sampling problem is formulated as a continuous-time Markov decision process with an uncountable state space. An exact solution to this problem is derived, which has a simple threshold-type structure. The threshold is time-invariant, regardless of the number of transmission failures since the last successful packet delivery. By expressing the threshold as the solution of a fixed-point equation, we can calculate the threshold by a low-complexity bisection search and fixed-point iterations. We find that, after a successful packet delivery, the optimal sampler may wait for a positive time period before taking the next sample and sending it out, whereas no waiting time should be added if the previous transmission failed. Numerical simulations are provided to compare different sampling policies. 

In this paper, we \textcolor{black}{aim to design an optimal sampler for a system} in which fresh samples of a signal (source) are sent through an unreliable channel to a remote estimator, and acknowledgments are sent back over a feedback channel. Both the forward and feedback channels could have random transmission times \textcolor{black}{due to time varying channel conditions}. Motivated by distributed sensing, the estimator can estimate the real-time value of the source signal by combining the signal samples received through the channel and \textcolor{black}{the} noisy signal observations collected from a local sensor. We prove that the estimation error is a non-decreasing function of the Age of Information (AoI) for \textcolor{black}{the} received signal samples and design an optimal sampling strategy that minimizes the long-term average estimation error subject to a sampling rate constraint. \textcolor{black}{The} sampling strategy is also optimal for minimizing the long-term average of general non-decreasing functions of the AoI. The optimal sampler design follows a randomized threshold strategy: If the last transmission was successful, the source waits until the expected estimation error upon delivery exceeds a threshold and then sends out a new sample. If the last transmission fails, the source immediately sends out a new sample without waiting. The threshold is the root of a fixed-point equation and can be solved with low complexity (e.g., by bisection search). The optimal sampling strategy holds for general transmission time distributions of the forward and feedback channels. Numerical simulations are provided to compare different sampling policies. 



\end{abstract}



\begin{IEEEkeywords}
Age of information, unreliable transmissions, two-way delay, \textcolor{black}{and sampling}.
\end{IEEEkeywords}







==> sections/backup.tex <==






\begin{comment}

\section{Proof of (30) and (34)}\label{appeq-discountedm}
%In Appendix~\ref{appeq-discountedm}, we provide the proof of \eqref{eq-totalsingle2} and \eqref{eq-discountedm}.
For the channel assumed to be reliable after $m-1$ consecutive failures, we have $P(M=k) = \alpha^{k-1} (1-\alpha) $ if $k=1,2,\cdots,m-1$, and $P(M=m) = \alpha^{m-1}$ (if $m=\infty$, then $P(M=k) = \alpha^{k-1}(1-\alpha)$ for all $k=1,2,\cdots$). The statement \eqref{eq-totalsingle2} is shown by taking $m=\infty$, and \eqref{eq-discountedm} is shown by taking $m=n$.
We have
\begin{align}
\nonumber & J^m_{\pi}(w) \\  \nonumber = &  \mathbb{E} \left[   \sum_{j=1}^{M} g(W_j,Z_{j})   \ \Big{|} \  W_1 = w \right]  \\
\nonumber = & \sum_{k = 1}^{m}  \mathbb{E} \left[ \sum_{j=1}^{M} g(W_j,Z_{j})   \ \Big{|} \  W_1 = w, M = k \right]
 \times \mathbb{P} (M = k) \\
 \nonumber
  \overset{(i)}{=} & \sum_{k = 1}^{m}  \mathbb{E} \left[ \sum_{j=1}^{k}  g(W_j,Z_{j})    \ \Big{|} \  W_1 = w  \right]  \times \mathbb{P} (M = k) \\
 \nonumber
= &  \sum_{j=1}^{m}   \sum_{k = j}^{m}  \mathbb{E} \left[  g(W_j,Z_{j})   \ \Big{|} \  \Delta_1 = w \right]  \times \mathbb{P} (M = k)  \\
= & \sum_{j=1}^{m} \alpha^{j-1} \mathbb{E} \left[  g(W_j,Z_{j})   \ \Big{|} \  \Delta_1 = \delta, X_1 = x \right].   
\end{align}
Because the decisions $Z_{j}$ $(j = 1,\ldots,k)$ are causal, thus $g(W_j,Z_{j})$ is independent of $M$ given that $M\ge j$. In other words, the decision $Z_j$ remains the same whether $M=j$ or $M=j+1,\ldots$ This validates step (i).
%Also, step $(ii)$ is due to Lemma \ref{lemma_boundedbelow} and the rearrangement of series in \cite[Chapter 3]{rudin1976principles}. 



\end{comment}

\begin{comment}

\section{An Alternative proof to Lemma~\ref{lemma-jw}}\label{appendix-lemma-jw}



We now turn to the case $|w| \ge v$. Since $\tau=0$, we have $X_\tau=w, J_{n+1}(w) = G_{n+1}(w)$ and
\begin{align}
J_{n+1}(w,y) & =\mathbb{E} \left[ Y \right] w^2+ \frac{1}{2} \mathbb{E} \left[ Y^2 \right] - \mathbb{E} \left[ Y \right] \text{mse}_{\text{opt}}  + \alpha \mathbb{E}_{W_{Y_1}} \left[   J_n(w + W_{Y_1}) \right], \\
% & = \mathbb{E} \left[ Y \right] w^2+ \frac{1}{2}\mathbb{E} \left[ Y^2 \right] - \mathbb{E} \left[ Y \right]\text{mse}_{\text{opt}} +y  + \alpha \mathbb{E}_{W_{Y_1}} \left[   g(w + W_{Y_1},\tau)  + \alpha^2 \mathbb{E} \left[   J(W_{(3)}) \right] \right]. 
\alpha \mathbb{E}_{W_{Y_1}} \left[   J_n (w + W_{Y_1}) \right] & = \alpha \mathbb{E} \left[   g(w + W_{Y_1},v_n) \right] +  \alpha^2 \mathbb{E} \left[   g(W_2(w),v_{n-1}) \right] + \cdots +  \alpha^n \mathbb{E} \left[   g(W_n(w),v_{1}) \right]. 
\end{align} Here $W_{n+1}(w)$ represents the state value after $n$ samples where the initial state is $w$.
We divide $W_{n+1}(w)$ into $n$ districts (cases). Only in the first case, $W_{n+1}(w)$ is the function of $w$, for the remaining cases, $W_{n+1}(w)$ is independent of $w$.   
\begin{align}
W_{n+1}(w) = \left\{
\begin{array}{lll}
w+W_{Y_1}+\cdots+W_{Y_{n+1}} & \  |w+W_{Y_1}|\ge v_n,\cdots |w+W_{Y_1}+\cdots+W_{Y_{n}}| \ge v_2 \vspace{1mm} \\
\pm v_2 + W_{Y_{n+1}} = W_2(\pm v_2) & \   |w+W_{Y_1}|\ge v_n, \cdots |w+W_{Y_1}+\cdots+W_{Y_{n}}| \le v_2 \vspace{1mm} \\
\cdots & \\
W_n(\pm v_n) &  |w+W_{Y_1}| \le v_n
\end{array}
\right.
\end{align}

Let us call each case case~$1$ to case~$n$ for simplicity.
Now we analyze $ \frac{d}{dw} \mathbb{E} \left[  J_{n+1}(w+W_Y) \right]$, i.e., we solve 
\begin{align}
\lim_{\Delta w \rightarrow 0} \frac{1}{\Delta w} \mathbb{E} \left[ J_{n+1}(w+\Delta w+W_Y) -  J_{n+1}(w+W_Y) \right].
\end{align}
 If both $w$ and $w+\Delta w$ are in the same case (this has close to $1$ probability), then\footnote{For the ease of description, We may use $g(w)$ to replace $g(w,v)$, because at each stage the threshold $v$ is fixed.} for case~$1$,    
\begin{align}
\nonumber & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w} \mathbb{E} \left[  \left( g(w+\Delta w+W_{Y_1}+\cdots+W_{Y_{n+1}}) - g(w+W_{Y_1}+\cdots+W_{Y_{n+1}}) \right)  {\text{\large $\mathbbm{1}$}}_{ c1(w),c1(w+\Delta w)}  \right]  \\
\nonumber = & \lim_{\Delta w \rightarrow 0}  \mathbb{E} \left[ \left( g'(w+W_{Y_1}+\cdots+W_{Y_{n+1}}) + o(\Delta w) \right) {\text{\large $\mathbbm{1}$}}_{ c1(w),c1(w+\Delta w)}  \right]\\
\nonumber = & \mathbb{E} \left[ g'(w+W_{Y_1}+\cdots+W_{Y_{n+1}}) {\text{\large $\mathbbm{1}$}}_{ c1(w)} \right]. %\\
%\nonumber = & \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right] X_{\sum_{k=1}^{n} Y_k} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{k=1}^{i-1} Y_k}|\ge v_{n+1-i}, i=2,3,...,n \right\} }   \\ & + \left( 2\beta X_{\sum_{k=1}^{n+1} Y_k} - \frac{2}{3} X^3_{\sum_{k=1}^{n+1} Y_k} \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{k=1}^{n+1} Y_k}| < v_{1},  |X_{\sum_{k=1}^{i-1} Y_k}|\ge v_{n+1-i}, i=2,3,...,n \right\} } \Bigg{]}.
\end{align}
The second equality is due to (i) Dominated convergence theorem and (ii) $P(c1(w) \cap c1^c(w+\Delta w) )\rightarrow 0$ from Lemma~\ref{lemma-prerequisite}(b).
For case~$2$ to case~$n$, due to the symmetric of $W_Y$, $g(W_n(v_n)) = g(W_n(-v_n)) $. So for $k=2,\cdots,n,$ 
\begin{align}
\nonumber & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w} \mathbb{E} \left[  \left( g(W_{n+1}(w+\Delta w)) - g(W_{n+1}(w)) \right)  {\text{\large $\mathbbm{1}$}}_{ ck(w),ck(w+\Delta w)}  \right] \\
 = & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w} \mathbb{E} \left[  \left( g(W_k(v_k)) - g(W_k(v_k)) \right)  {\text{\large $\mathbbm{1}$}}_{ ck(w),ck(w+\Delta w)}  \right]=0. \label{eq-case2n0}
\end{align}
The analysis of \eqref{eq-case2n0} and continuity of $g(\cdot)$ also can show that $J_{n+1}(v_{n+1}-) = J_{n+1}(v_{n+1})$ (by setting $w = v_{n+1}$ and setting $\Delta w <0, \Delta w \rightarrow 0-$).
If $w$ and $w+\Delta w$ are not in the same case, we want to show that the gap vanishes to zero. Suppose that it gets from case~$k1$ to case~$k2$. For simplicity, suppose that $k_1<k_2$. Then, $k_1$ is the least index that $|w+\Delta w +W_{Y_1}+\cdots W_{Y_{k_1}}| <v_{k_1}$. Note that the policy is a fixed hitting time, so the only randomness lies in the evolution of increment $\{ W_t,t\ge 0 \}$ for each stopping time $\tau_1,\cdots,\tau_{n+1}$ with $t=0$ as the starting point, and the random value $W_{Y_1},\cdots,W_{Y_n+1}$. These randomness are mutually independent. For different initial states $w$ and $w+\Delta w$, we couple the same randomness. Then, after the $k1$th sample, with probability (call the event as $A$\footnote{The event $A$ is defined as: at each stage $k$ with $v_k>0$, after the stopping time that either case $w$ or case $w+\Delta w$ first exceeds the threshold, the Wiener evolution of the remaining case cannot reach $\pm |\Delta w|$ before reaching $ \mp (2v_k - |\Delta w|)$, which has at least $1 -  \Delta w / (2v -  \Delta w)  -  \Delta w / (2v -  \Delta w) $ probability, which closes to $1$. Under event $A$, it always holds that $0 \le W_{n+1}(w+\Delta w) - W_{n+1}(w) \le \Delta w$. Event $A$ guarantees that $W_{n+1}(w+\Delta w) - W_{n+1}(w)$ is a contraction mapping in $n$. Due to the strong Markov property of the Wiener process, $A$ is quite simple and is independent of $W_{Y_k}$'s and any evolution of stopping times at each stage. }) at least $(1- \Delta w/v_{k_1})^n = 1-O(\Delta w)$\footnote{If $v_{k+1}=0$, then case~$k_1$ has zero probability, thus can be neglected.}, which closes to $1$,
%The event $A$ is defined as: For $k1,\cdots, n$, if either the two states enters within the threshold, then after the stopping time, the two states share the same threshold and are still within at most $\Delta w$. The event $A^c$ is thus defined as: there exits a sample index in $k1,\cdots, n$, if either the two states enters within the threshold, then after the stopping time, the two states becomes opposite threshold value. An alternative definition of $A$ is: $\{ 0 \le W_{n+1}(w+\Delta w) - W_{n+1}(w) \le \Delta w \}$. This event has at least  probability $(1-\Delta w /v)^n $, which closes to $1$, and $v$ is the minimum value of at most $n$ non-zero thresholds. 
\begin{align}
\Delta w>0: \ 0 \le W_{n+1}(w+\Delta w) - W_{n+1}(w) \le \Delta w, \\
\Delta w<0: \ \Delta w \le W_{n+1}(w+\Delta w) - W_{n+1}(w) \le 0.
 \end{align}  
Since $g(\cdot)$ is continuously differentiable almost surely, $g(W_{n+1}(w))$ is continuous and $W_{n+1}(w) \approx W_{n-k_1}(\pm v_{k_1})$. Also, $P(ck_1(w), ck_1^c (w+\Delta w)) $ is linear in $\Delta w$ and canceled out by $1/\Delta w$. Without loss of generality, assume $W_{k1}(w) \approx v_{k1}$ and thus $W_{k1}(w+\Delta w) = W_{k1}(w) + \Delta w$. We have 
\begin{align}
\nonumber & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w} \mathbb{E} \left[  \left( g(W_{n+1}(w+\Delta w)) - g(W_{n+1}(w)) \right)  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w),A}  \right]. \\ 
\nonumber = & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w} \mathbb{E} \left[  g'(W_{n-k1}( v_{k1}) +\epsilon) \Delta w {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w), A}   \right] \\
 = & \lim_{\Delta w \rightarrow 0} \mathbb{E} \left[  g'(W_{n-k1}( v_{k1}) +\epsilon) {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w), A}   \right]
=0.
\end{align}
The last equality is from Dominated convergence theorem and the fact that ${\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w), A} \le {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w)} \rightarrow 0$ almost surely. 
Also, the event $A$ is related to the evolution of the wiener process after a stopping time at each stage (the stopping time may be zero), and thus is independent of $W_{1},\cdots,W_{Y_{n+1}}$ (i.e., $A$ is independent of the partitioned events $c1(w),\cdots,cn(w)$), $A$ has probability $1 - n \Delta w/v$ closing to $1$, and we have 
\begin{align}
\nonumber & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w} \mathbb{E} \left[  \left( g(W_{n+1}(w+\Delta w)) - g(W_{n+1}(w)) \right)  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w),A^c}  \right]. \\ 
%\nonumber \le  & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w} \mathbb{E} \left[ 2g(|v_{k1}| +|W_{Y_{k1}}|+\cdots+|W_{n+1}| + |\Delta w|)  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w), A^c}   \right] \\
\nonumber =  & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w}  \mathbb{E} \left[ {\text{\large $\mathbbm{1}$}}_{A^c} \right] \mathbb{E} \left[ g(W_{n+1}(w+\Delta w)) - g(W_{n+1}(w))  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w)}  | A^c \right] \\
  \le   & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w}  \mathbb{E} \left[ {\text{\large $\mathbbm{1}$}}_{A^c} \right] \mathbb{E} \left[  2g( w + \max\{ v_{1},\cdots,v_n \} +|W_{Y_{1}}|+\cdots+|W_{n+1}| + |\Delta w|)  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w)}   | A^c \right] 
  \\
  =   & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w}  \mathbb{E} \left[ {\text{\large $\mathbbm{1}$}}_{A^c} \right] \mathbb{E} \left[  2g( w + \max\{ v_{1},\cdots,v_n \} +|W_{Y_{1}}|+\cdots+|W_{n+1}| +  |\Delta w|)  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w)}  \right]  \\
    \le   & \lim_{\Delta w \rightarrow 0} b \mathbb{E} \left[  2g( w + \max\{ v_{1},\cdots,v_n \} +|W_{Y_{1}}|+\cdots+|W_{n+1}| + 1)  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w)}  \right] \\
%    \le   & \lim_{\Delta w \rightarrow 0}  \frac{1}{\Delta w}  \mathbb{E} \left[ {\text{\large $\mathbbm{1}$}}_{A^c} \right] \mathbb{E} \left[ 2 \left(\max_{k1\le k \le n} \{v_{k}\} +|W'_{Y_{k1}}|+\cdots+|W'_{n+1}| +1 \right)^2  {\text{\large $\mathbbm{1}$}}_{ ck_1(w),ck_2(w+\Delta w)}  \right] \\
= & 0, 
\end{align} where $b$ is a constant. %Here, we define $W'_Y$ as the truncated variable of $W_Y$ given that $|W_Y| \ge \max_{k1\le k \le n} \{v_{k}\}$.

In conclusion, for all $n$, 
\begin{align}
\nonumber & \frac{d}{d w} \mathbb{E} \left[ J_{n+1} (w+W_Y) \right] \\ 
\nonumber = & \lim_{\Delta w \rightarrow 0} \frac{1}{\Delta w} \mathbb{E} \left[ J_{n+1}(w+\Delta w+W_Y) -  J_{n+1}(w+W_Y) \right]\\
 \nonumber = & \lim_{\Delta w \rightarrow 0}  \sum_{j=1}^{n+1} \alpha^{j-1}  \frac{1}{\Delta w} \mathbb{E} \left[  \left( g(w+\Delta w+W_{Y_1}+\cdots+W_{Y_{n+1}}) - g(w+W_{Y_1}+\cdots+W_{Y_{n+1}}) \right)  {\text{\large $\mathbbm{1}$}}_{ c1(w),c1(w+\Delta w)}  \right] \\
  = &   \sum_{j=1}^{n+1} \alpha^{j-1}  \mathbb{E} \left[ g'(w+W_{Y_1+\cdots +Y_{j}}) {\text{\large $\mathbbm{1}$}}_{ |w+W_{Y_1}| \ge v_{n+1},\cdots, |w+W_{Y_1+\cdots +Y_{j-1}}| \ge v_{n+3-j}  } \right]  \label{eq-dwjny} \\
  \nonumber  = &  \sum_{j=1}^{n+1} \alpha^{j-1}   \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right] X_{\sum_{k=1}^{n} Y_k} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{k=1}^{i-1} Y_k}|\ge v_{n+1-i}, i=2,3,...,n \right\} }   \\ 
  & + \left( 2\beta X_{\sum_{k=1}^{n+1} Y_k} - \frac{2}{3} X^3_{\sum_{k=1}^{n+1} Y_k} \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{k=1}^{n+1} Y_k}| < v_{1},  |X_{\sum_{k=1}^{i-1} Y_k}|\ge v_{n+1-i}, i=2,3,...,n \right\} } \Bigg{]}. 
 \label{eq-dwjny2}
\end{align}
The equations \eqref{eq-dwjny},\eqref{eq-dwjny2} imply that $J_{n+1}(v_{n+1}+) = J_{n+1}(v_{n+1})$. Combined with $J_{n+1}(v_{n+1}-) = J_{n+1}(v_{n+1})$, $J_{n+1}(w)$ is continuous at $ \pm v_{n+1}$ and thus continuous at everywhere.
Note that function $g_{n+1}(w)$ is differentiable except $\pm v_{n+1}$, but $g_{n+1}(w)$ is continuous and the incident $|w+W_{Y}+\cdots + W_{Y_{n}}| =a$ has zero measure, so $g_{n+1}'(\pm v_{n+1})$ can choose in arbitrary sequel. Note that 
\begin{align}
\nonumber \frac{d}{d w} J_{n+1} (w) & =  \frac{d}{d w} g_{n+1} (w)  + \alpha  \frac{d}{dw} \mathbb{E} \left[   J_n(w+W_{Y_2}) \right] {\text{\large $\mathbbm{1}$}}_{ |w| \ge v_{n+1}  }    \\
\nonumber & =  2 \mathbb{E} \left[ Y \right] w {\text{\large $\mathbbm{1}$}}_{ |w| \ge v_{n+1}  } + ( 2 \text{mse}_{\text{opt}} w - \frac{2}{3} w^3 ) {\text{\large $\mathbbm{1}$}}_{ |w| < v_{n+1}  } + \alpha  \frac{d}{dw} \mathbb{E} \left[   J_n(w+W_{Y_2})   \right]  {\text{\large $\mathbbm{1}$}}_{ |w| \ge v_{n+1}  }  \\
  & =  \sum_{j=1}^{n+1} \alpha^{j-1} \mathbb{E} \left[  g'(w+W_{Y_2+\cdots +Y_{j}}) {\text{\large $\mathbbm{1}$}}_{ |w|\ge v_{n+1}, |w+W_{Y_2}| \ge v_{n},\cdots, |w+W_{Y_2+\cdots +Y_{j-1}}| \ge v_{n+3-j}  }  \right].\label{eq-jn1wder1}
\end{align}
Then, we replace $w$ by $w+W_{Y_1}$, and take expectation on $W_{Y_1}$, comparing to \eqref{eq-dwjny}, gets  
\begin{align}
 \mathbb{E} \left[  \frac{d}{dw}  J_n(w+W_Y) \right] =  \frac{d}{dw} \mathbb{E} \left[   J_n(w+W_Y) \right]. 
\end{align}
In addition, by \eqref{eq-jn1wder1}, continuity of $\mathbb{E} \left[  g'(w+W_{Y_2+\cdots +Y_{j}}) {\text{\large $\mathbbm{1}$}}_{ |w|\ge v_{n+1}, |w+W_{Y_2}| \ge v_n,\cdots, |w+W_{Y_2+\cdots +Y_{j-1}}| \ge v_2  }  \right]$ by Lemma~\ref{lemma-prerequisite}(b) and the continuity of $g'(w,v_{n+1})$ for all $w$ except at $w = \pm v_{n+1}$, $J'_{n+1}(w)$ is continuous for all $w$ except at $w = \pm v_{n+1}$, by the definition of $v_{n+1}$ in Lemma~\ref{derivative1}, we find that $J_{n+1}'( \pm v_{n+1})$ is still continuous.   



\end{comment}












\begin{comment}

\section{Others}

Note that the state evolution of the stopping time $\tau$ satisfies
\begin{align}
|W_{n+1}|\le \max \{ |W_n|,v \} +|W_{Y_n}| \le |W_n|+v+|W_{Y_n}|. 
\end{align}
Therefore, 
\begin{align}
|W_{n+1}|\le |w|+  n v+ \sum_{j=1}^{n} |W_{Y_j}|. 
\end{align}
Then, since $Y_j$'s are i.i.d. and $\mathbb{E} \left[ Y^2 \right]<\infty$, for any given value $w$, each single cost satisfies 
\begin{align}
\alpha^n |  \mathbb{E} \left[ g(W_{n+1},\tau) \right] | \le \alpha^n   \mathbb{E} \left[ Y \right] \mathbb{E} \bigg[   \Big{(} |w|+  n v+ \sum_{j=1}^{n} |W_{Y_j}| \Big{)}^2 \bigg] + \alpha^n b = O(\alpha^n n^2), \label{eq-cost1bound}
\end{align}
where $b$ is a bounded value that is not related to $w$ and $n$. Note that $ \alpha^n n^2 \rightarrow 0$ and $\sum_{n=1}^{\infty} \alpha^n n^2 <\infty$. So we have $\tilde{J}_n(w,y)\rightarrow \tilde{J}(w,y)$ for any given $w,y$. 

Also, from\eqref{eq-cost1der1}, \eqref{eq-cost1der2}, $2\beta X_{\sum_{j=1}^{n} Y_j} - \frac{2}{3} X_{\sum_{j=1}^{n} Y_j}^3$ is bounded given that $ |X_{\sum_{j=1}^{n} Y_j}|\le v$. So we have
\begin{align}
 \frac{d}{dw} \alpha^n \mathbb{E} \left[ g(W_{n+1},\tau)  \right] \le \alpha^n \mathbb{E} \left[ Y \right] \mathbb{E} \left[ 2 |X_{\sum_{j=1}^{n} Y_j} |  \right] +\alpha^i b_1 = O(\alpha^n n), \label{eq-cost1derbound}
\end{align}
where $b_1$ is a bounded value that is not related to $w$ and $n$.
Similarly, $\sum_{n=1}^{\infty} \alpha^n n <\infty$, and $\partial / \partial w\tilde{J}_n(w,y)$ converges for all given $w,y$. Since $\partial / \partial w \tilde{J}_n(w,y)$ converges, and $\tilde{J}_n(w,y)$ converges to $\tilde{J}(w,y)$, utilizing \cite[Theorem~7.17]{rudin1976principles}, $\partial / \partial w \tilde{J}_n(w,y)$ converges to $\partial / \partial w \tilde{J}(w,y)$, i.e., 
\begin{align}
& \tilde{J}_w (w,y) \\ \triangleq & \frac{\partial }{\partial w} \sum_{n=1}^{\infty} \alpha^{n-1} \mathbb{E} \left[ g(W_n,\tau) \right] \\  = &  \sum_{n=1}^{\infty} \alpha^{n-1} \frac{d }{d w}  \mathbb{E} \left[ g(W_n,\tau) \right]\\ % =  \sum_{j=1}^{\infty} \alpha^{j-1}  \mathbb{E} \left[ \frac{\partial }{\partial w} g(W_j,\tau) \right]. 
 = & 2 \mathbb{E} \left[ Y \right] w +
\sum_{n=1}^{\infty} \alpha^n \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right] X_{\sum_{j=1}^{n-1} Y_j} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} }   \\ & + \left( 2\beta X_{\sum_{j=1}^{n} Y_j} - \frac{2}{3} (X_{\sum_{j=1}^{n} Y_j})^3 \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} } \Bigg{]}.
\end{align}
In other words, we can replace the derivation with summation.
This ends our proof.

\end{comment}

\begin{comment}
\begin{align}
f'(w) = & \frac{2}{3} w^3 - 2\beta w +
\sum_{n=1}^{\infty} \alpha^n \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right] X_{\sum_{j=1}^{n-1} Y_j} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} }   \\ & + \left( 2\beta X_{\sum_{j=1}^{n} Y_j} - \frac{2}{3} (X_{\sum_{j=1}^{n} Y_j})^3 \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} } \Bigg{]},
\end{align}
where $X_0 = w$. Since $f(w)$ is a even function, $f'(0)=0$. By Definition~\ref{def-optimalpi}, $f'(v)=0$. Since $f(v)=0$, we want to show that $f'(w) \le 0$ for $0\le w \le v$. 

Using the same analysis in the proof of Lemma~\ref{derivative1}, we get 
\begin{align}
f''(w) = & 2 w^2 - 2\beta  +
\sum_{n=1}^{\infty} \alpha^n \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right]  {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} }   \\ & + \left( 2\beta  - 2 (X_{\sum_{j=1}^{n} Y_j})^2 \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} } \Bigg{]}. \label{eq-fxx} \\
f'''(w) = & 4w +
\sum_{n=1}^{\infty} \alpha^n \mathbb{E} \bigg{[}   \left(  - 4 X_{\sum_{j=1}^{n} Y_j} \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} } \bigg{]}. \\
f''''(w) = & 4 +
\sum_{n=1}^{\infty} \alpha^n \mathbb{E} \bigg{[}    - 4 \times {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} } \bigg{]}. \label{eq-fxxxx}
\end{align}
Note that the summation of probabilities
\begin{align}
& \sum_{n=1}^\infty \alpha^n \times P  \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} \\  
<  & \sum_{n=1}^\infty P  \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} \\
= & 1,
\end{align} where the last equality holds because the events $ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\}_{n=1,2,\cdots}$ are disjoint and complementary.
\end{comment}

\begin{comment}

%We now turn to the case $|w| \ge v$. Since $\tau=0$, we have $X_\tau=w$ and
%\begin{align}
%\tilde{J}(w,y) & =\mathbb{E} \left[ Y \right] w^2+ \frac{1}{2} \mathbb{E} \left[ Y^2 \right] - \mathbb{E} \left[ Y \right] \text{mse}_{\text{opt}} +y  + \alpha \mathbb{E}_{W_{Y_1}} \left[   J(w + W_{Y_1}) \right]\\
% & = \mathbb{E} \left[ Y \right] w^2+ \frac{1}{2}\mathbb{E} \left[ Y^2 \right] - \mathbb{E} \left[ Y \right]\text{mse}_{\text{opt}} +y  + \alpha \mathbb{E}_{W_{Y_1}} \left[   g(w + W_{Y_1},\tau)  + \alpha^2 \mathbb{E} \left[   J(W_{(3)}) \right] \right]. 
%\end{align}
The state value $W_{(3)}$ comes from the initial state value $X_{Y_1}\triangleq w+W_{Y_1}$ undergoing the hitting time $\tau$ and a random delay $W_{Y_2}$.
We first focus on the term $\alpha  \mathbb{E} \left[   g(w + W_{Y_1},\tau) \right] $. Note that $P(|w+W_{Y_1}=v|)=0$. So we have almost surely, 
\begin{align}
\frac{d}{dw} g(w+W_{Y_1},\tau)  = \left\{
\begin{array}{lll}
2 \mathbb{E} \left[ Y \right] (w+W_{Y_1}) & \  |w+W_{Y_1}|\ge v, \vspace{1mm} \\
-\frac{2}{3} (w+W_{Y_1})^3 + 2(\beta+\mathbb{E} \left[ Y \right])(w+W_{Y_1})  & \ |w+W_{Y_1}|<v.
\end{array}
\right.
\end{align}
%Similar to the analysis in \eqref{eq-cost1smalldv1}---\eqref{eq-cost1smalldv4}, we have almost surely,
%\begin{align}
% J'(w+W_{Y_1}) = \tilde{J}_x(w+W_{Y_1},0) = \frac{d}{dw}g(w+W_{Y_1},\tau) + \alpha\times \left\{
%\begin{array}{lll}
%  \frac{d}{dw} \mathbb{E}_{w_{Y_2}} \left[   J(w+W_{Y_1+Y_2}) \right]  & \  |w+W_{Y_1}| \ge v, \vspace{1mm} \\
% 0 & \ |w+W_{Y_1}|<v.
%\end{array}
%\right.
%\end{align}
%So we get (if $|w| \ge v$):
%\begin{align}
%\tilde{J}_w(w,y) | W_c = 2cw + \alpha \times  \left\{
%\begin{array}{lll}
%2c(w+W_c) + \alpha \frac{d}{dw} \mathbb{E}_{w_{c2}} \left[   J(w+W_{2c}) \right]  & \  |w+W_c| \ge v, \vspace{1mm} \\
%-\frac{2}{3} (w+W_c)^3 + 2(\beta+c)(w+W_c)+0 & \ |w+W_c|<v.
%\end{array}
%\right.
%\end{align}
Since $\mathbb{E} \left[ Y^2 \right]<\infty$, $\mathbb{E} \left[ |W_{Y}|^n \right]<\infty$ for $n=1 \cdots 4$. Utilizing Dominated convergence theorem, $\frac{d}{dw}  \mathbb{E} \left[   g(w + W_{Y_1},\tau) \right] = \mathbb{E} \left[  \frac{d}{dw} g(w + W_{Y_1},\tau) \right] $. So if $|w| \ge v$,
\begin{align}
\tilde{J}_w(w,y)  =  &2 \mathbb{E} \left[ Y \right] w + \alpha \frac{d}{dw}  \mathbb{E}_{w_{Y_1}} \left[   J(w+W_{Y_1})  \right] \label{eq-cost0and1} \\
= & 2 \mathbb{E} \left[ Y \right] w +  \alpha \frac{d}{dw} \mathbb{E}_{W_{Y_1}} \left[   g(w + W_{Y_1},\tau) \right]  + \alpha^2  \frac{d}{dw} \mathbb{E} \left[   J(W_{(3)}) \right]  \\
= &  2 \mathbb{E} \left[ Y \right] w +  \alpha \mathbb{E}_{W_{Y_1}} \left[  \frac{d}{dw}  g(w + W_{Y_1},\tau) \right]  + \alpha^2  \frac{d}{dw} \mathbb{E} \left[   J(W_{(3)}) \right]  \\
                          =  &2  \mathbb{E} \left[ Y \right] w +
 \alpha \times  \mathbb{E} \left[  2 \mathbb{E} \left[ Y \right] w + \left(  2\beta X_{Y_1} - \frac{2}{3} X_{Y_1}^3 \right) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| < v} \right]  + \alpha^2 \frac{d}{dw}  \mathbb{E} \left[   J(W_{(3)})  \right]  \label{eq-cost0and1and2} 
\end{align}
Here, we have set $X_t$ as a Wiener process with $X_0=w$, so $X_{Y_1} = w+W_{Y_1}$.
If $|w|\ge v$ and $|X_{Y_1}|<v$, 
\begin{align}
%& W_3 = \left(w+W_{Y_1+Y_2} \right) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| \ge v} \\
& W_{(3)} = \left\{
\begin{array}{lll}
v+W_{Y_2} & \ \text{with probability } \frac{v+X_{Y_1}}{2v}, \vspace{1mm} \\
-v+W_{Y_2}  & \ \text{with probability } \frac{v-X_{Y_1}}{2v}.
\end{array}
\right.
\end{align} Therefore,
\begin{align}
& \alpha^2 \frac{d}{dw}  \mathbb{E} \left[   J(W_{(3)})  \right]  = 
\alpha^2 \frac{d}{dw}  \mathbb{E} \left[   J  \left(w+W_{Y_1+Y_2} \right) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| \ge v}  \right] \label{eq-cost1and2} \\
 & + \alpha^2 \frac{d}{dw} \mathbb{E}_{Y_1} \left[  \frac{v+X_{Y_1}}{2v} \times  \mathbb{E}_{Y_2} \left[ J(v+W_{Y_2}) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| < v} \right] +  \frac{v-X_{Y_1}}{2v} \times  \mathbb{E}_{Y_2} \left[ J(-v+W_{Y_2}) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| < v} \right] \right]. \label{eq-cost2} \\
  = &
\alpha^2 \frac{d}{dw}  \mathbb{E} \left[   J  \left(w+W_{Y_1+Y_2} \right) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| \ge v}  \right]  + \alpha^2 \frac{d}{dw} \mathbb{E}_{Y_1} \left[   \mathbb{E}_{Y_2} \left[ J(v+W_{Y_2})  \right] {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| < v}  \right].
\end{align} Note that $J(\pm v+W_{Y_2})$ is not related to $w$, and for any $|X_{Y_1}| \ne v$, there exists an $\epsilon>0$ such that ${\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| < v} = {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1} \pm \epsilon | < v}$. Thus, almost surely,  
\begin{align}
\frac{d}{dw} J(\pm v+W_{Y_2}) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| < v} =0, \label{eq-cost2is0}
\end{align}also, by Dominated convergence theorem, the terms in \eqref{eq-cost2} is zero.
This statement combined with \eqref{eq-cost1and2},\eqref{eq-cost2}, we have
\begin{align}
 \alpha^2 \frac{d}{dw}  \mathbb{E} \left[   J(W_{(3)})  \right]  = 
\alpha^2 \frac{d}{dw}  \mathbb{E} \left[   J  \left(w+W_{Y_1+Y_2} \right) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| \ge v}  \right] + \alpha^2 (f_{Y_1}(-v-w) - f_{Y_1}(v-w)) \mathbb{E}_{Y_2} \left[ J(v+W_{Y_2})  \right]
\end{align}
The above equation and \eqref{eq-cost0and1and2} imply that 
\begin{align}
\tilde{J}_w(w,y) =  &2  \mathbb{E} \left[ Y \right]  w +
 \alpha \times  \mathbb{E} \left[  2 \mathbb{E} \left[ Y \right] w + \left(  2\beta X_{Y_1} - \frac{2}{3} X_{Y_1}^3 \right) {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| < v} \right] \\ 
 & + \alpha^2 \frac{d}{dw}  \mathbb{E}_{w_{Y_1},w_{Y_2}} \left[   J(w+W_{Y_1+Y_2})  {\text{\large $\mathbbm{1}$}}_{ |X_{Y_1}| \ge v}  \right]. \label{eq-cost0and1and2and3}
\end{align}
We look at \eqref{eq-cost0and1},\eqref{eq-cost0and1and2and3} and iterate for multiple times. Let us denote $\tilde{J}_n(w,y) = y+ \sum_{i=0}^{n} \alpha^i \mathbb{E}^{w,y} \left[ g(W_{i+1},\tau)  \right] $ as the discounted cost of $n+1$ samples, $n\ge1$.
Under $n-1$ iterations after \eqref{eq-cost0and1},\eqref{eq-cost0and1and2and3}, we get the following results for the cost of $n+1$th sample and $\tilde{J}_n(w,y)$:
\begin{align}
& \frac{d}{dw} \alpha^n \mathbb{E} \left[ g(W_{n+1},\tau)  \right]  =  \alpha^n    \times \mathbb{E} \Bigg{[}  2 c X_{\sum_{j=1}^{n-1} Y_j} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} }  \label{eq-cost1der1}  \\ & + \left( 2\beta X_{\sum_{j=1}^{n} Y_j} - \frac{2}{3} (X_{\sum_{j=1}^{n} Y_j})^3 \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} } \Bigg{]}, \label{eq-cost1der2}\\ 
& \tilde{J}_n(w,y) = \sum_{i=0}^{n} \frac{d}{dw} \alpha^i \mathbb{E} \left[ g(W_{i+1},\tau)  \right]  = 2 \mathbb{E} \left[ Y \right] w + \sum_{i=1}^{n} \alpha^i
 \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right] X_{\sum_{j=1}^{i-1} Y_j} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,i \right\} }   \\ & + \left( 2\beta X_{\sum_{j=1}^{i} Y_j} - \frac{2}{3} (X_{\sum_{j=1}^{i} Y_j})^3 \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{i} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,i \right\} } \Bigg{]}.
\end{align}

\end{comment}


==> sections/bio.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/Jiayu.eps}}]{Jiayu Pan} received the B.S. degree in Physics from Shanghai Jiao Tong University, Shanghai, China in 2017. He is currently pursuing the Ph.D. degree with the Electrical and Computer Engineering Department, at the Ohio State University, OH, USA. His research interests include wireless communication and age of information. He received the First Prize Scholarship from Shanghai Jiao Tong University in 2015.    
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/Ahmed.eps}}]{Ahmed M. Bedewy} received the B.S. and M.S. degrees in electrical and electronics engineering from Alexandria University, Alexandria, Egypt, in 2011 and 2015, respectively, and the Ph.D. degree in electrical and computer engineering from The Ohio State University, OH, USA, in 2021. His research interests include wireless communication, cognitive radios, resource allocation, communication networks, information freshness, optimization, and scheduling algorithms. He received the Awarded Certificate of Merit and First Class Honors for being
one of the top ten undergraduate students, for the period 2006–2008, and the First, for the period 2008–2011, in electrical and electronics engineering. His article received the runner-up for the Best Paper Award of ACM MobiHoc 2020.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/Yin-Sun.eps}}]{Yin Sun}  (Senior Member, IEEE) is currently an Assistant Professor with the Department of Electrical and Computer Engineering, Auburn University. He received his B.Eng. and Ph.D. degrees in electronic engineering from Tsinghua University in 2006 and 2011, respectively. From 2011 to 2017, he was a Post-Doctoral Scholar and a Research Associate with The Ohio State University. His research interests include wireless networks, age of information, machine learning, robotic control, and information theory. He co-authored a monograph \emph{Age of Information: A New Metric for Information Freshness} (Morgan and Claypool Publishers, 2019). He has been a Guest Editor of the \emph{IEEE Journal on Selected Areas in Communications} for the special issue on ``Age of Information in Real-time Systems and Networks," a Guest Editor of \emph{Entropy} for the special issue on ``Age of Information: Concept, Metric and Tool for Network Control," a Guest Editor of \emph{Frontiers in Communications and Networks} for the special issue on ``Age of Information," an Associate Editor of the \emph{IEEE Transactions on Network Science and Engineering}, and an Editor of the \emph{Journal of Communications and Networks}. His articles received the Best Student Paper Award from the IEEE/IFIP WiOpt 2013, the Best Paper Award from the IEEE/IFIP WiOpt 2019, runner-up for the Best Paper Award of ACM MobiHoc 2020, and the 2021 \emph{Journal of Communications and Networks (JCN)} Best Paper Award. He received the Auburn Author Award in 2020. He co-founded the Age of Information Workshop in 2018. He is a member of the ACM.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1.1in,height=1.3in]{figures/shroff.eps}}]{Ness B. Shroff} (S’91–M’93–SM’01–F’07)
received the Ph.D. degree in electrical engineering from Columbia University in 1994. 
He joined Purdue University immediately thereafter as an Assistant Professor with the School of Electrical and 
Computer Engineering.  At Purdue, he became a Full Professor of ECE and the director of a university-wide center on wireless systems and 
applications in 2004. In 2007, he joined The Ohio State University, where he holds the Ohio Eminent Scholar Endowed Chair in 
networking and communications, in the departments of ECE and CSE. He holds or has held visiting (chaired) professor positions at Tsinghua 
University, Beijing, China, Shanghai Jiaotong University, Shanghai, China, and IIT Bombay, Mumbai, India. He has received numerous best paper awards for his 
research and is listed in Thomson Reuters’ on The World’s Most Influential Scientific Minds, and is noted as a Highly Cited Researcher by Thomson Reuters. He currently serves as the steering committee chair for ACM Mobihoc and the Editor in Chief of the IEEE/ACM Transactions on Networking. He received the IEEE INFOCOM Achievement Award for seminal contributions to scheduling and resource allocation in wireless networks.  
\end{IEEEbiography}

==> sections/introduction_backup.tex <==

\section{Introduction}\label{introduction}

Timely updates are crucial in many applications such as vehicular networks, wireless sensor networks, and UAV navigations. To achieve timely updates, we require the destination to receive fresh information from the remote source as quickly as possible. The information freshness is measured by age of information, or simply age, which has been widely explored in recent years (e.g., \cite{bedewy2019agee,bedewy2019minimizing,sun2018age,bedewy2019age,bedewy2021low,pan2021minimizing,zouminimizing,qian2020minimizing,yates2021age,sun2017remote,ornee2019sampling,tsai2020unifying,huang2020real,yates2015lazy,sun2017update,sun2019sampling,tsai2020age,tsai2021jointly,arafa2020timely,klugel2019aoi,pan2021minimizings,kaul2012real}). Age of information with the function of current time $t$ is defined as $\Delta_t = t-U_t$, where $U_t$ is the generation time of the freshest information data. %An early study in \cite{kaul2012real} has characterized the difference between age and some well-known metrics such as delay and throughput. In an elementary queuing system, higher throughput suggests more frequent status update, but leads to a destination receiving higher delayed updates; lower throughput implies less frequent update and leads to the information staleness.
In several different \textcolor{black}{queueing} systems, the Last-Generated, First-Served (LGFS) policy is shown to achieve age-optimality \cite{bedewy2019agee,bedewy2019minimizing,sun2018age}. Scheduling policies in various wireless networks are studied to minimize age  \cite{bedewy2019age,bedewy2021low,pan2021minimizing,zouminimizing,qian2020minimizing}.   
A literature review of \textcolor{black}{recent works} in age of information is provided in \cite{yates2021age}.

In \cite{sun2017remote} and \cite{ornee2019sampling}, a connection between age of information and remote estimation of time-varying processes (e.g., Wiener process or Ornstein-Uhlenbeck (OU) process) was established. One of the remote estimation objectives in these early studies \textcolor{black}{was} to design an optimal sampling policy to minimize the long-term average minimum mean square error (MMSE).
The MMSE is a function of \textcolor{black}{the} age if the sampling policy is independent of the signal being sampled \cite{tsai2020unifying,sun2017remote,ornee2019sampling,huang2020real}. %However, the destination can receive not only the delayed signal data, but also an instant noisy observation from the source. 
Among these studies, the estimator obtains the exact signal samples subject to delay. However, the estimator neglects the instant and inexact signal samples.  
For example, in vehicular networks, the estimator can estimate a signal via both the exact signal samples from the remote sensor and the instant camera streaming from the close vehicle sensor over time.  
%However, the results are based on the assumption that the estimator can only observe the staled data, but not the real-time noisy linear side information. 
To consider both the delayed and instant signal samples, we will apply the Kalman Filter \textcolor{black}{\cite[Chapter 7]{poor2013introduction}} and study the relationship between the MMSE and age of information. 
%without using the knowledge of the observed OU process.     

%A common sampling policy for a generate-at-will source is the zero-wait policy; it sends the fresh data whenever the previous sample is delivered and can minimize delay and maximize throughput. However, to reduce the age, the source needs to wait before submitting a new sample \cite{yates2015lazy}. The study in \cite{sun2017update} generalizes the result in \cite{yates2015lazy} 
%and derives the optimal sampling policy under a general function of age and general channel delay distribution. The results imply that the zero-wait policy is far from optimal if the channel delay is heavy-tailed.    
%In \cite{tsai2020age}, the authors extends the results by considering a two-way delay where both the forward direction and the backward (feedback) direction have a random delay. 
The desire for timely updates and the study of the new remote estimation problem \textcolor{black}{necessitates considering general non-linear age functions in the development of optimal sampling policies.} 
To reduce the age, we may require the source to wait before submitting a new sample, i.e., the zero-wait policy may not be age-optimal\footnote{We refer to a policy as \emph{zero-wait} if the source generates the sample and transmits as soon as it receives the acknowledgement.} \cite{yates2015lazy}. The study in \cite{sun2017update} generalized the result in \cite{yates2015lazy}, proposed an optimal sampling policy under a Markov channel with sampling rate constraint, and observed that the zero-wait policy is far from optimal if, for example, the transmission times are heavy-tail distributed or positively correlated.     
In \cite{sun2019sampling}, the authors provided a survey of the age penalty functions related to autocorrelation, remote estimation, and mutual information. The optimal sampling solution is a deterministic or randomized threshold policy based on the objective value and the sampling rate constraint. %However, the studies in \cite{sun2017update,sun2019sampling} assume reliable transmissions. Moreover, they consider a one-way transmission delay and ideally assume that the backward direction has a zero delay. 
However, in real-time network systems, both the forward direction and the feedback direction have a random delay. Such a random two-way delay model was considered in e.g., \cite{tsai2020age,tsai2021jointly}.        
In \cite{tsai2020age}, the paper proposed a low complexity algorithm with a quadratic convergence rate to compute the optimal threshold.  
In \cite{tsai2021jointly}, an optimal joint cost-and-AoI minimization solution was provided for multiple coexisting source-destination pairs with heterogeneous AoI penalty functions. 
Although the above studies have \textcolor{black}{developed optimal} sampling strategies, they assume that the transmission process is reliable. However, due to the channel fading, the channel conditions are time-varying, and thus the transmission process is unreliable. %In addition, 

\textcolor{black}{Recent studies \cite{arafa2020timely,klugel2019aoi} investigate sampling strategies while considering} unreliable transmissions. %but with a constant one-way delay. 
In \cite{arafa2020timely}, the authors considered quantization errors, noisy channel, and non-zero receiver processing time, and they established the relationship between the MMSE and age. For general age functions, they provided optimal sampling policies, given that the sampler needs to wait before receiving feedback. When the sampler does not need to wait, they \textcolor{black}{provided} enhanced sampling policies that perform better than previous ones.  %However, using convex optimization is incorrect (even for a constant delay) if we allow the sampling policy to be randomized. 
In \cite{klugel2019aoi}, the authors chose \emph{idle} or \emph{transmit} at each time slot to minimize joint age penalty and transmission cost. The optimality of a threshold-based policy is shown, and the policy's threshold is computed efficiently. %Nevertheless, the technique of \cite{klugel2019aoi} is infeasible in our study since we consider an enlarged action space and random channel delays. 
Nevertheless, in practice, transmission delays are random rather than constant because of \textcolor{black}{congestion}, random sample sizes, etc, \textcolor{black}{which is a critical challenge facing the design of sampling strategies.} 


\textcolor{black}{To address the aforementioned challenges, we investigate how to design optimal sampling strategies} in wireless networks under the following more realistic (and general) conditions that have largely been unexplored: unreliable transmissions and random delay in both forward and feedback directions. %In this aspect of studying optimal sampling, comprehensive comparisons between existing literature and our study are relegated to Section \ref{related}.                  
%In this paper, we focus on designing an optimal sampling policy on minimizing a general function of age assuming unreliable transmissions and random two-way delay. 
Early studies on optimizing sampling assuming reliable channels with random delays %\cite{sun2017update,sun2019sampling,tsai2020age,tsai2020unifying,sun2017remote,ornee2019sampling} 
have shown that the sampling problem is decomposed into a per-sample problem. The per-sample problem can be further solved by optimization theory (e.g., \cite{yates2015lazy,sun2017update,sun2019sampling,tsai2020age}) or optimal stopping rules (e.g., \cite{tsai2020unifying,sun2017remote,ornee2019sampling}). 
Similarly, our problem assuming an unreliable channel is equivalent to a per-epoch problem containing multiple samples until successful packet delivery.
Therefore, the per-epoch problem is a Markov Decision Process (MDP) with an uncountable state space, which is \textcolor{black}{a} key difference with past works, (e.g., \cite{yates2015lazy,sun2017update,sun2019sampling,tsai2020age,tsai2020unifying,sun2017remote,ornee2019sampling}) and faces the curse of dimensionality.\footnote{\textcolor{black}{We further compare our technical differences with past works in Section~\ref{discussion}}.}
The main contributions of this paper are stated as follows:        

%which can be solved explicitly using Karush–Kuhn–Tucker (KKT) conditions

\begin{itemize}

\item We first formulate the problem where the estimator estimates a signal in real-time by combining noisy signal observations from a local sensor and accurate signal samples received from a remote sensor. 
We show that if the sampling policy is made independently of the signal being sampled, the MMSE equals an increasing function of the age of \textcolor{black}{the} received signal samples.  

\item For general nonlinear age functions, or simply age penalty functions, we provide an exact solution for minimizing these data freshness metrics.  
The optimal sampling policy has a simple threshold-type structure, and the threshold can be efficiently computed by bisection search and fixed-point iterations. We uncover the following interesting property: if the last transmission is successful, the optimal policy may wait for a positive time period before generating the next sample and sending it out; otherwise, no waiting time should be added. The key technical approach developed in our results is given as follows: (i) The value function of the proposed policy is an exact solution to the Bellman equation. (ii) Under the contraction mapping assumption, the solution to the Bellman equation is unique, which guarantees optimality of our proposed threshold-based policy. %(iii) The Lagrangian dual problem and strong duality \cite{bertsekas2003convex} determine the threshold of the optimal policy. 
Our results hold for (i) general non-decreasing age penalty functions, (ii) general delay distributions of both the forward and feedback channels, (iii) sampling problems both with or without a sampling rate constraint. Therefore, our paper extends previous studies on sampling for optimizing age (e.g., \cite{yates2015lazy,sun2017update,sun2019sampling,tsai2020age,arafa2020timely,klugel2019aoi}). Although our sampling problem is \textcolor{black}{in} continuous time, it can be easily reduced to be in discrete time.

\item When there is no sampling rate constraint, we provide \textcolor{black}{necessary and sufficient conditions on the optimality of the zero-wait sampling policy \cite{yates2021age}} based on the choice of age penalty function, forward and feedback channels. 
Finally, numerical simulations show that our optimal policy can reduce the age compared with other approaches. 

\end{itemize}


%The rest of the paper is organized as follows: In Section \ref{related}, we discuss some related works. In Section \ref{estimation}, we describe our system model and the result of remote estimation. In Section \ref{section-system}, we formulate our sampling problem for general age penalty functions. We then present our main results for the optimal sampling problem in Section \ref{main}. The proof sketches of the main results are provided in Section \ref{section-proof}. Numerical simulations are provided to validate our results in Section \ref{numerical}. Finally, we summarize our contributions in Section \ref{conclusion}.  



==> sections/plan.tex <==
\section{plan}
\begin{itemize}

\item Title: Sampling Wiener Process for Remote Estimation under Unreliable Transmissions: Extension to Age of Information. Authors: myself, prof. Sun, and prof. Shroff.

\item Introduction: Despite quite a few works have been working on, process aware sampling problem is still a challenging problem. We will proceed further from reliable channel to possibly unreliable channel and positively random channel delay. This extension poses challenges because we need to consider a multiple samples stopping problem instead of single sample stopping time problem. Although one previous work has solved with process ignorant cases, the decision predicts the evolution of the age and thus not a stopping time. We use value iteration algorithms, in each iteration, we show the exact solution. The physical meaning of the value iteration at $n$th step is quite intuitive: we provide the optimal stopping times $\tau^*_1,\cdots,\tau^*_n$ where the channel state condition is i.i.d., at previous $n-1$ transmissions, but the $n$th transmission must succeed. Under the convergence assumption, the optimal policy is provided in theorem~4.   


\item Main Result: 

\begin{proposition}\label{prop-aware}
There exists an optimal policy in $\Pi_{\text{signal-aware}}$ such that $\{ S_{i+1,M_{i+1}} - S_{i,M_i} \}_i$ are i.i.d. Moreover, our original problem is equivalent to
\begin{align}
\text{mse}_{\text{opt}} = & \inf_{\pi \in \Pi_i} \frac{ \mathbb{E} \left[  \int_{D_{i-1,M_{i-1}}}^{D_{i,M_i}} (W_t - W_{S_{i-1,M_{i-1}}})^2 dt \right]}{ \mathbb{E} \left[   D_{i,M_i} - D_{i-1,M_{i-1}} \right] }. \label{prop1eq}
\end{align} 
\end{proposition}

\begin{theorem}
An optimal solution to problem \eqref{prop1eq} is:
\begin{align}
 & S_{i,1}(\beta) =  \inf_{t}  \left\{  t\ge D_{i-1,M_{i-1}}(\beta):  
 | W_t - \hat{W}_t |    \ge v  \right\}, \\  
 & S_{i,j}(\beta) =  \inf_{t}  \left\{  t\ge D_{i,j-1}(\beta):  
 | W_t - \hat{W}_t |    \ge v  \right\}, \ j=2,3,\ldots,
\end{align}
the optimal threshold $v$ is the root of 
\begin{align}
0 = & \frac{2}{3} v^3 - 2\beta v +
\sum_{n=1}^{\infty} \alpha^n \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right] X_{\sum_{j=1}^{n-1} Y_j} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} }   \\ & + \left( 2\beta X_{\sum_{j=1}^{n} Y_j} - \frac{2}{3} X^3_{\sum_{j=1}^{n} Y_j} \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v,  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v, k=2,3,...,n \right\} } \Bigg{]}. 
\end{align}
${\text{\large $\mathbbm{1}$}}_A$ is the indicator function of event $A$, $X_t$ is the wiener process with $X_0=v$, $ \text{mse}_{\text{opt}} = \beta+\mathbb{E} \left[ Y \right]$ is the solution to 
\begin{align}
 \text{mse}_{\text{opt}} = \frac{ \mathbb{E} \left[  \int_{D_{i-1,M_{i-1}}(\beta)}^{D_{i,M_{i}}(\beta)} (W_t - \hat{W}_t)^2 dt \right]}{ \mathbb{E} \left[ D_{i,M_{i}} - D_{i-1,M_{i-1}} \right] }. \label{eq-betafraction}
\end{align}
\end{theorem}


\item Proof of Theorem~4:

\begin{definition} Denote $\pi_j^*$ as the stopping time for the $j$th sample. Suppose that the current state value is $w$. 
\begin{align}
\pi_j^*  = \inf_{t\ge 0}\{t:  |w+W_t|\ge v_j  \},
\end{align}
$v_1 = \sqrt{3\beta}$,

$v_j$ $(j=2,3\cdots)$ is the root of 
\begin{align}
0 = & \frac{2}{3} v^3 - 2\beta v +
\sum_{n=1}^{j} \alpha^n \mathbb{E} \Bigg{[}  2 \mathbb{E} \left[ Y \right] X_{\sum_{j=1}^{n-1} Y_j} {\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{k-1} Y_j}|\ge v_{j-k+1}, k=2,3,...,n \right\} }   \\ & + \left( 2\beta X_{\sum_{j=1}^{n} Y_j} - \frac{2}{3} X^3_{\sum_{j=1}^{n} Y_j} \right){\text{\large $\mathbbm{1}$}}_{ \left\{ |X_{\sum_{j=1}^{n} Y_j}| < v_{j-n+1},  |X_{\sum_{j=1}^{k-1} Y_j}|\ge v_{j-k+1}, k=2,3,...,n \right\} } \Bigg{]}, 
\end{align}
$X_t$ is the wiener process with $X_0=v_j$


\end{definition}
Denote $J^{j}_{\pi}(w)$ as the discounted cost of $j$ samples, such that the first sample chooses policy $\pi$, and the remaining samples follow policy $\pi_{j-1}^*,\pi_{j-2}^*\cdots \pi_{1}^*$. Then we have the following backward induction properties:
\begin{proposition}\label{prop-valueiteration}
We have
 $TJ^j_{\pi_j^*} = J^j_{\pi_j^*}$, i.e., 
\begin{align}
& J_{\pi_1^*}(w) = \inf_{\tau} g_\tau(w), j=1, \label{eq-bellmann1} \\
& J_{\pi_j^*}(w) = \inf_{\tau} g_\tau(w)+ \alpha \mathbb{E} \left[ J_{\pi_{j-1}^*} (\text{the next state value}) \right], j=2,3,...
\end{align}
\end{proposition}









\end{itemize}



==> sections/problem_form.tex <==


%\title{Problem Formulation}
%	\title{Detection of Spatial Sparsity in Cognitive Radio Networks based on Compressive Sensing}


% \maketitle
% ------------------------------ ABSTRACT -----------------------------
\section{System Model}
\begin{figure}[t]
\includegraphics[scale=.5]{figures/Sys_mod.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{System model.}
%\vspace{-.09in} 
 \label{sys_mod}
\end{figure}
We consider a remote estimation system as illustrated in Fig. \ref{sys_mod}, where a sensor takes samples from Ornstein-Uhlenbeck (OU) process $X_t$ and forwards the samples to an estimator via an error-free channel. Besides, the estimator has a continuous time noisy observation of the process $X_t$, called $O_t$. The error-free channel is modeled as a FCFS queue with i.i.d. service times. We suppose that there is an acknowledgement that is sent back to the sampler with zero delay whenever a sample is delivered. 

The System starts to operate at time $t=0$. We use $S_i$ to denote the generation time of the $i$-th sample, while $D_i$ denote  its delivery time to the estimator. Moreover, we use $Y_i$ to denote the service time of the $i$-th sample, where we have $0<\mathbb{E}[Y]<\infty$ and $D_i=S_i+Y_i$. Let $U(t)=\max{S_i:D_i\leq t}$ be the
sampling time of the latest received sample at time $t$. The age of information, or simply age, at time $t$ is defined as 
\begin{equation}
\Delta(t)=t-U(t).
\end{equation}
Since we have $D_{i}\leq D_{i+1}$, $\Delta(t)$ can be expressed as
\begin{equation}
\Delta(t)=t-S_i, \text{if}~t\in[D_i,D_{i+1}), i=0,1,2,\ldots
\end{equation}

The considered OU process  is defined as the solution to the following stochastic differential equation  (SDE)
\begin{equation}
dX_t=-\theta X_t dt+W_t,
\end{equation}
where $\theta>0$ is a parameter, and $W_t$ is a zero mean white noise process such that we have $\mathbb{E}[W_tW_s]=Q\delta(t-s)$ for all $0\leq t,s\leq\infty$. The observation process $O_t$ is modeled as 
\begin{equation}
O_t=HX_t+V_t,
\end{equation}
Where $H$ is some constant and $V_t$ is a zero mean white noise process such that we have $\mathbb{E}[V_tV_s]=R\delta(t-s)$ for all $0\leq t,s\leq\infty$.  We suppose that $W_t$ and $V_t$ are uncorrelated such that we have $\mathbb{E}[W_tV_s]=0$ for all $0\leq t,s\leq\infty$.

In this work, we use the Kalman filter \cite{ poor2013introduction} as the estimator. The Kalman filter provides an estimate $\hat{X}_t$ at time $t$. We aim to seek the optimal sampler that minimizes the mean-squared estimation (MSE) error $P_t\triangleq\mathbb{E}[(X_t-\hat{X}_t)^2]$  subject to an average sampling-rate constraint, which can be cast as the following problem:
\begin{align}
\text{mse}_\text{opt}=&\inf_{\pi\in\Pi}\limsup_{T\to\infty}\frac{1}{T}\mathbb{E}\left[\int_{0}^T P_t dt\right]\label{opt_eq5}\\&
\text{s.t.} \liminf_{n\to \infty}\frac{1}{n}\mathbb{E}\left[\sum_{i=1}^n (S_{i+1}-S_i)\right]\geq\frac{1}{f_\text{max}},\label{opt_eq6}
\end{align}
where $\text{mse}_\text{opt}$ is the optimum value of \eqref{opt_eq5}, $f_\text{max}$ is the maximum allowed sampling rate, and $\Pi$  represents the set of all causal sampling policies (some condition might be needed here such as regenerative condition, etc.). Note that the objective function in \eqref{opt_eq5} can be rewritten as (due to the regenerative property and renewal theory):
\begin{equation}
\limsup_{T\to\infty}\frac{1}{T}\mathbb{E}\left[\int_{0}^T P_t dt\right]=\limsup_{n\to\infty}\frac{\mathbb{E}\left[
\sum_{i=0}^n\int_{D_i}^{D_{i+1}} P_t dt\right]}{\mathbb{E}[D_n]}.
\end{equation}

The estimation process works as follows: The Kalman filter uses the continuous time observation $O_t$ to estimate the process $X_t$. Once a sample $i$ is delivered to the Kalman filter at time $D_i$, the Kalman filter re-initiate itself with the initial condition $P_{S_i}=0$ and starts a new estimation session. According to \cite{ poor2013introduction}, $P_t$ for $t
\in[D_i,D_{i+1})$ satisfies the following Riccati differential equation:
\begin{align}
\frac{dP_t}{dt}=-2\theta P_t+Q-\frac{H^2}{R}P_t^2.\label{rec_eqn}
\end{align}
Next, we derive a solution for Equation \eqref{rec_eqn} and show that $P_t$ is a non-decreasing function of the age process $\Delta(t)$.
\section{Main Results}
Let us define $\bar{P}$ as the steady state solution of \eqref{rec_eqn}, i.e., it is the solution of the following equation:
\begin{align}
0=-2\theta P_t+Q-\frac{H^2}{R}P_t^2.\label{rec_eqn_st}
\end{align}
Since our model is observable and controllable, we have $\bar{P}>0$. Hence, $\bar{P}$ is given by
\begin{align}
\bar{P}=\frac{-\theta R+\sqrt{(\theta R)^2+QRH^2}}{H^2}.
\end{align}
We derive $P_t$ in the next lemma.
\begin{lemma}\label{lim1}
For $t\in[D_i,D_{i+1})$ and $ i=0,1,2,\ldots$, the MSE $P_t$ is given by
\begin{align}
P_t=\bar{P}-\frac{1}{\frac{H^2}{2\sqrt{(\theta R)^2+QRH^2}}+\left(\frac{H^2}{-\theta R+\sqrt{(\theta R)^2+QRH^2}}-\frac{H^2}{2\sqrt{(\theta R)^2+QRH^2}}\right)e^{2\sqrt{\theta+Q\frac{H^2}{R}}\Delta(t)}}, \label{Lem1eq}
\end{align}
where $\Delta(t)=t-S_i$. Moreover, $P_t$ is a non-decreasing function of the age $\Delta(t)$.
\end{lemma}
\begin{proof}
See Appendix \ref{Appendix_A}.
\end{proof}
As a result of Lemma \ref{lim1}, we can use \cite{sun2017update} directly to solve our sampling Problem. Next, we show that when there is no side observation, i.e., $O_t=0$ for  $t\ge 0$, then our sampling problem reduces to the signal-agnostic sampling problem that is studied in \cite{ornee2019sampling}.
\begin{lemma}\label{Lim2}
When $O_t=0$ when $t\geq 0$, then the MSE $P_t$ for $t\in[D_i, D_{i+1})$ and $i=0,1,2 ,\ldots$ is given by
\begin{align}
P_t=\frac{Q}{2\theta}\left(1-e^{-2\theta\Delta(t)}\right).\label{Lim2_eq}
\end{align}
\end{lemma}
\begin{proof}
See Appendix \ref{Appendix_B}.
\end{proof}
Lemma \ref{Lim2} agrees with \cite[Lemma 4]{ornee2019sampling}.


%\bibliographystyle{IEEEbib}
%\bibliography{MyLib}
%\section{Appendix}
%\appendices





==> sections/related.tex <==
\section{Related Works}\label{related}


%Further, when the source process is the Wiener process, the expected square estimation error is equal to the age of information \cite{sun2020sampling}. 
%These imply that sampling for minimizing the estimation error can be equivalent to sampling for minimizing a function of the age of information.

Our paper is closely related to the research area of the age of information. 
Age of information, or simply age, is a metric to evaluate data freshness. Age has gained much popularity in the recent decade and has contributed to various remote control systems such as sensor networks, UAV navigation, and semantic communication. Age at current time $t$ is defined as $\Delta(t) = t - U(t)$, where $U(t)$ is the generation time of the latest delivered sample. A recent literature review on the age is provided in \cite{yates2021age}.

When the sampling times are independent of a Wiener source process, the expected square estimation error is equal to the age \cite{sun2020sampling}. Thus, our study contributes to sampling for minimizing the age, e.g., in \cite{arafa2021timely,arafa2020age,sun2019sampling,pan2022optimal,moltafet2022status,hui2022real}. In \cite{arafa2021timely}, the paper studies sampling energy harvesting sources with a unit battery buffer under an erasure channel. In the case of a single source, it provides an optimal sampling policy without feedback. With perfect feedback, an optimal policy is offered among the policies that may wait only when the previous transmission is successful. In \cite{arafa2020age}, the paper solves explicit optimal solutions for an energy harvesting source with finite buffer sizes, where the arrived energy can fill up the whole buffer or fill up incrementally.     
In \cite{sun2019sampling}, the authors relate autocorrelation, remote estimation, and mutual information to the nonlinear age penalty functions, and provide an optimal sampling policy under sampling rate constraint. %The optimal policy performs much better than the zero-wait policy if the transmission delay is heavy-tailed.  
In \cite{pan2022optimal}, when the source process is a multidimensional Gaussian diffusion process, and the estimator is the Kalman Filter, the expected square estimation error is an increasing function of the age. For a general non-decreasing age penalty function, the optimal sampling policy has a threshold structure under unreliable channel conditions and random transmission delay. An extended sampling scenario where the sampler can transmit the sample before receiving the feedback is studied in \cite{moltafet2022status}. 

==> sections/system.tex <==

%\section{Model and Formulation}\label{section-system}
%\section{Problem Formulation for Age Penalty}\label{section-system}
%\section{Problem Formulation for General Age Penalty}\label{section-system}

% i.e., $S_{i,j}$ assigns a probability measure on $[A_{i,j},\infty)$ based on $\mathcal{H}_{i,j}$. %Specifically, we call a policy in $\Pi$ is stationary if $Z_{i,j}$ is parameterized only by current state $\delta_{i,j}$. We call a policy is deterministic if $p(dz_{i,j} | \delta_{1,1},z_{1,1},y_{1,1},\delta_{1,2}...\delta_{i,j})$ assigns mass one to a point. 
%We assumed that the total cost in each epoch is finite, i.e.,
%\begin{equation}\label{fenzi-finite}
%\mathbb{E} \left[  \int^{D_{i,M_i}}_{D_{i-1,M_{i-1}}}  p(\Delta_t) dt \right] < \infty.
%\end{equation}
%We assume that any sampling policy in the collection $\Pi$ has the following assumptions:  
%Further, we assume that $T_i= S_{i,M_i}-S_{i-1,M_{i-1}}$ is a regenerative process: there exists an increasing sequence $0\le k_1 < k_2< \ldots$ of finite random variables such that the post-$k_j$ process $\{ T_{k_j+i},i=0,1,\ldots \} $ has the same distribution as the post-$k_1$ process  $\{ T_{k_1+i},i=0,1,\ldots \}$ and is independent of the pre-$k_j$ process $ \{ T_i, i=1,2, \ldots, k_j-1 \}$; in addition, $\mathbb{E} \left[  k_{j+1}-k_j \right]<\infty$, $\mathbb{E} \left[  S_{k_1,M_{k_1}} \right]<\infty$ and $0<\mathbb{E} \left[  S_{k_{j+1},M_{k_{j+1}}}-S_{k_j,M_{k_j}} \right]<\infty$, $j=1,2, \ldots$\footnote{ In this paper, we will optimize $\limsup_{T\rightarrow \infty} (1/T) \mathbb{E} \left[  \int_{0}^{T} p(\Delta_t) dt \right]$. However, a nicer objective is to optimize $ \lim_{n\rightarrow \infty}  \mathbb{E} \left[  \int^{D_{n,M_n}}_{0}  p(\Delta_t) dt \right] $ $/ \mathbb{E} \left[  D_{n,M_n}  \right] $. If $T_i$ is a regenerative process, then the two objective functions are equal \cite{haas2006stochastic}, \cite{gallager2013stochastic}. If no conditions are applied, they are different.}  


%Recent works such as \cite{arafa2020timely,sun2019sampling} also omit the constraint on the waiting time.

   
 


Here, $C(T)$ is the total number of samples taken by time $T$, and $f_{\text{max}}$ is the maximum allowed sampling rate. The constraint \eqref{avg-constraint} is added because in practice, the sensor may need to keep working for a long time with limited amount of energy.  
To avoid triviality, the optimal objective value $p_{\text{opt}}$ in \eqref{avg} satisfies $p_{\text{opt}}<\bar{p}$, where $\bar{p}=\lim_{\delta\rightarrow \infty} p(\delta)$. Note that we allow $\bar{p}$ to be infinite. 


%Note that we have removed the cases that $Z_{i,j}<0$, i.e., sample a packet and store in the queue before delivery. 
%This is because such a policy can be replaced by a policy that samples at exact delivery time and remains the same average age performance. See \cite{sun2017remote,sun2017update,ornee2019sampling,sun2019sampling}. 


%\Delta_{\text{opt}}





